DePLOI: Applying NL2SQL to Synthesize and Audit Database Access Control

In every enterprise database, administrators must define an access control policy that specifies which users have access to which tables. Access control straddles two worlds: policy (organization-level principles that define who should have access) and process (database-level primitives that actually implement the policy). Assessing and enforcing process compliance with a policy is a manual and ad-hoc task. This paper introduces a new access control model called Intent-Based Access Control for Databases (IBAC-DB). In IBAC-DB, access control policies are expressed using abstractions that scale to high numbers of database objects, and are traceable with respect to implementations. This paper proposes DePLOI (Deployment Policy Linter for Organization Intents), a LLM-backed system leveraging access control-specific task decompositions to accurately synthesize and audit access control implementation from IBAC-DB abstractions. As DePLOI is the first system of its kind to our knowledge, this paper further proposes IBACBench, the first benchmark for evaluating the synthesis and auditing capabilities of DePLOI. IBACBench leverages a combination of current NL2SQL benchmarks, real-world role hierarchies and access control policies, and LLM-generated data. We find that DePLOI achieves high synthesis accuracies and auditing F1 scores overall, and greatly outperforms other LLM prompting strategies (e.g., by 10 F1 points).

==> tables/audit_prompting.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llllll}
\hline
Auditing  & CoT  & Least-to-Most & Few-Shot & Self-Consistency & Persona \\ \hline
Precision & 0.98 & 0.94          & 1.0      & 0                & 1.0     \\
Recall    & 0.75 & 1.0           & 0.76     & 0                & 0.013   \\
F1 Score  & 0.85 & 0.96          & 0.86     & --               & 0.026   \\ \hline
\end{tabular}%
}
\caption{\nameofsys\ Auditing Prompting Strategy Choice}
\label{tab:audit-prompt}
\end{table}

==> tables/fullsummary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
                                                                      & \multicolumn{1}{l}{Plain LLM} & \multicolumn{1}{l}{Sentence} & \multicolumn{1}{l}{Word} & \multicolumn{1}{l}{Jaccard} & \multicolumn{1}{l}{LLM4AC} \\ \midrule
\begin{tabular}[c]{@{}l@{}}NL vs NL\\ Total\\ RV 1-F1\end{tabular}    & 0.149                         & 0.084                        & 0.220                    & 0.204                       & \textbf{0.041}             \\
\begin{tabular}[c]{@{}l@{}}NL vs NL\\ Total\\ Priv 1-F1\end{tabular}  & 0.119                         & 0.116                        & 0.122                    & 0.116                       & \textbf{0.003}             \\
\begin{tabular}[c]{@{}l@{}}NL vs SQL\\ Total\\ RV 1-F1\end{tabular}   & 0.553                         & 0.765                        & 0.632                    & 0.837                       & \textbf{0.035}             \\
\begin{tabular}[c]{@{}l@{}}NL vs SQL\\ Total\\ Priv 1-F1\end{tabular} & 0.021                         & 0.007                        & 0.014                    & 0.014                       & \textbf{0.006}             \\ \bottomrule
\end{tabular}%
}
\caption{LLM4AC Differencer F1 Errors across
all DBs and Perturbations. Lower is better.}
\label{tab:fullresults}
\end{table}

==> tables/llmnl2sql.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llllllll@{}}
\toprule
\textbf{Method} & \textbf{Metric} & \begin{tabular}[c]{@{}l@{}}Admin Only\\ Read\end{tabular} & \begin{tabular}[c]{@{}l@{}}Admin Only\\ Read/Write\end{tabular} & \begin{tabular}[c]{@{}l@{}}Complex \\ RBAC\end{tabular} & DAC  & \begin{tabular}[c]{@{}l@{}}Complex \\ RBAC\\ + Views\end{tabular} & \begin{tabular}[c]{@{}l@{}}DAC\\ + Views\end{tabular} \\ \midrule
\textbf{Naive}  & \textbf{Syntax} & 0.11                                                      & 0.11                                                            & 0.16                                                    & 0.09 & 0.06                                                              & 0.05                                                  \\
\textbf{Rolled} & \textbf{Syntax} & 0.23                                                      & 0.18                                                            & 0.15                                                    & 0.24 & 0.13                                                              & 0.11                                                  \\
\textbf{C3}     & \textbf{Syntax} & 1                                                         & 1                                                               & 1                                                       & 1    & 1                                                                 & 1                                                     \\
\textbf{Naive}  & \textbf{FRF}    & 0.06                                                      & 0.04                                                            & 0.07                                                    & 0.05 & 0.01                                                              & 0.02                                                  \\
\textbf{Rolled} & \textbf{FRF}    & 0                                                         & 0.02                                                            & 0.04                                                    & 0.08 & 0.03                                                              & 0.01                                                  \\
\textbf{C3}     & \textbf{FRF}    & 1                                                         & 1                                                               & 0.89                                                    & 0.76 & 0.85                                                              & 0.69                                                  \\ \bottomrule
\end{tabular}%
}
\caption{Comparison of NL2SQL Translation by LLM method, with respect to syntax and Forward-Reverse-Forward (FRF) Accuracy. Columns are types of access control policies.}
\label{tab:llmnl2sql}
\end{table}

==> tables/nlvsnlsociome.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
Perturbation      & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Dr. Spider\\ Avg. RV F1\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Sociome\\ RV F1\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Dr. Spider\\ Avg. Priv F1\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Sociome\\ Priv F1\end{tabular}} \\ \midrule
column\_attribute & \textbf{0.951}                                                                      & 0.929                                                                       & 1.0                                                                                   & 1.0                                                                           \\
column\_value     & \textbf{0.985}                                                                      & 0.815                                                                       & 1.0                                                                                   & 1.0                                                                           \\
column\_synonym   & \textbf{0.937}                                                                      & 0.159                                                                       & \textbf{1.0}                                                                          & 0.8                                                                           \\
column\_carrier   & \textbf{0.989}                                                                      & 0.846                                                                       & 1.0                                                                                   & 1.0                                                                           \\
role\_syn         & 0.979                                                                               & \textbf{1.0}                                                                & 1.0                                                                                   & 1.0                                                                           \\
roledesc\_replace & 0.984                                                                               & \textbf{1.0}                                                                & 1.0                                                                                   & 1.0                                                                           \\
priv\_syn         & 0.998                                                                               & \textbf{1.0}                                                                & 1.0                                                                                   & 0.774                                                                         \\
priv\_inf         & 0.986                                                                               & \textbf{1.0}                                                                & \textbf{0.979}                                                                        & 0.774                                                                         \\ \bottomrule
\end{tabular}%
}
\caption{NL vs NL Role-View Mapping (RV) and Privilege Subsumption (Priv) F1 Scores on the Sociome DB vs Average F1 Scores over the Dr. Spider DBs.}
\label{tab:nlvsnlsociome}
\end{table}

==> tables/nlvssqlsociome.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
Perturbation      & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Dr. Spider\\ Avg. RV F1\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Sociome\\ RV F1\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Dr. Spider\\ Avg. Priv F1\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Sociome\\ Priv F1\end{tabular}} \\ \midrule
column\_attribute & \textbf{0.952}                                                                      & 0.519                                                                       & 1.0                                                                                   & 1.0                                                                           \\
column\_value     & \textbf{0.788}                                                                      & 0.462                                                                       & 1.0                                                                                   & 1.0                                                                           \\
column\_synonym   & \textbf{0.991}                                                                      & 0.159                                                                       & 1.0                                                                                   & 1.0                                                                           \\
column\_carrier   & \textbf{0.954}                                                                      & 0.519                                                                       & 1.0                                                                                   & 1.0                                                                           \\
role\_syn         & 0.993                                                                               & \textbf{1.0}                                                                & 1.0                                                                                   & 1.0                                                                           \\
roledesc\_replace & 0.968                                                                               & \textbf{1.0}                                                                & 1.0                                                                                   & 1.0                                                                           \\
priv\_syn         & \textbf{0.987}                                                                      & 0.519                                                                       & 0.958                                                                                 & \textbf{1.0}                                                                  \\
priv\_inf         & \textbf{0.994}                                                                      & 0.519                                                                       & 0.969                                                                                 & \textbf{1.0}                                                                  \\ \bottomrule
\end{tabular}%
}
\caption{NL vs SQL Role-View Mapping (RV) and Privilege Subsumption (Priv) F1 Scores on the Sociome DB vs Average F1 Scores over the Dr. Spider DBs.}
\label{tab:sociomenlvssql}
\end{table}

==> tables/sociomefull.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
Perturbation      & \begin{tabular}[c]{@{}l@{}}NL vs NL\\ Sociome\\ RV F1\end{tabular} & \begin{tabular}[c]{@{}l@{}}NL vs NL\\ Sociome\\ Priv F1\end{tabular} & \begin{tabular}[c]{@{}l@{}}NL vs SQL\\ Sociome\\ RV F1\end{tabular} & \begin{tabular}[c]{@{}l@{}}NL vs SQL\\ Sociome\\ Priv F1\end{tabular} \\ \midrule
column\_attribute & 0.929                                                              & 1.0                                                                  & 0.519                                                               & 1.0                                                                   \\
column\_value     & 0.815                                                              & 1.0                                                                  & 0.462                                                               & 1.0                                                                   \\
column\_synonym   & 0.159                                                              & 0.8                                                                  & 0.159                                                               & 1.0                                                                   \\
column\_carrier   & 0.846                                                              & 1.0                                                                  & 0.519                                                               & 1.0                                                                   \\
role\_syn         & 1.0                                                                & 1.0                                                                  & 1.0                                                                 & 1.0                                                                   \\
roledesc\_replace & 1.0                                                                & 1.0                                                                  & 1.0                                                                 & 1.0                                                                   \\
priv\_syn         & 1.0                                                                & 0.774                                                                & 0.519                                                               & 1.0                                                                   \\
priv\_inf         & 1.0                                                                & 0.774                                                                & 0.519                                                               & 1.0                                                                   \\ \bottomrule
\end{tabular}%
}
\caption{Role-View Mapping (RV) and Privilege
Subsumption (Priv) F1 Scores on the Sociome Policy}
\label{tab:diffsociome}
\end{table}

==> tables/synthres.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\footnotesize
\begin{tabular}{lr}
\toprule
Query Type                       & Accuracy  \\ \midrule
Single column Projection         & 50 / 50   \\
Multiple column Projection       & 50 / 50   \\
Single Whole-table Aggregation   & 30 / 30   \\
Single join                      & 50 / 50   \\
Multi-way join                   & 10 / 20   \\
Common Table Expression          & 40 / 40   \\
Nested Queries                   & 0 / 10    \\
Single WHERE clause condition    & 50 / 50   \\
Multiple WHERE clause conditions & 30 / 30   \\
Total Accuracy                   & 310 / 330 \\ \bottomrule
\end{tabular}%
\caption{LLM4AC Synthesizer Accuracy. The only errors were nested queries and multi-way joins.}
\label{tab:synthres}
\end{table}
